Bringing AI to the edge: A formal M&S specification to deploy effective IoT architectures

The Internet of Things is transforming our society, providing new services that improve the quality of life and resource management. These applications are based on ubiquitous networks of multiple distributed devices, with limited computing resources and power, capable of collecting and storing data from heterogeneous sources in real-time. To avoid network saturation and high delays, new architectures such as fog computing are emerging to bring computing infrastructure closer to data sources. Additionally, new data centers are needed to provide real-time Big Data and data analytics capabilities at the edge of the network, where energy efficiency needs to be considered to ensure a sustainable and effective deployment in areas of human activity. In this research, we present an IoT model based on the principles of Model-Based Systems Engineering defined using the Discrete Event System Specification formalism. The provided mathematical formalism covers the description of the entire architecture, from IoT devices to the processing units in edge data centers. Our work includes the location-awareness of user equipment, network, and computing infrastructures to optimize federated resource management in terms of delay and power consumption. We present an effective framework to assist the dimensioning and the dynamic operation of IoT data stream analytics applications, demonstrating our contributions through a driving assistance use case based on real traces and data.

==> text/annex_msg.tex <==
The message structure model is a simplified version of the one
proposed by the \gls{OSI} network model.

At a high level, information between nodes is transferred via
application messages. They only contain information about the
application, and their structure is the following:
\begin{itemize}
	\item \texttt{size}: size (in bits) of the application message. It
	models the amount of information contained by the message.
	\item \texttt{data}: data sent in the application message. Its
	content varies depending on the application message type.
	\item \texttt{packet\_id}: unique identifier for the application
	message. It is used for avoiding duplicates among the received
	messages.
\end{itemize}

For sending messages from one node to another, application messages
are encapsulated into network messages. Network messages contain
information about the node that generated the application message and
the node that is to receive the message. Their structure is the
following:
\begin{itemize}
	\item \texttt{node\_from}: node that generated and sent the
	message.
	\item \texttt{node\_to}: node that has to receive the message.
	\item \texttt{header}: size (in bits) of the network message
	header. It models the amount of information required for sending
	information from one node to another.
	\item \texttt{data}: application message to be sent.
	\item \texttt{packet\_id}: unique identifier of the network
	message.
\end{itemize}

The node that generated an application message and the one that is to
receive it may not be connected to the same network  – e.g.,
\glspl{UE} and \glspl{EDC} are not directly connected, but interact
with each other via \glspl{AP}. Network messages are sent within
physical messages. Physical messages depend on the environmnent
(optical fiber, wireles...), and provide point-to-point communication.

Physical messages contain the following fields:
\begin{itemize}
	\item \texttt{node\_from}: node that sent the message.
	\item \texttt{node\_to}: node that has to receive the message. It
	must be connected to the same network as \texttt{node\_from}.
	\item \texttt{header}: size (in bits) of the physical message
	header.
	\item \texttt{data}: this field contains the network message to be
	sent between nodes.
	\item \texttt{channel}: physical channel used for sending the
	message.
	\item \texttt{bandwidth}: bandwidth (in Hz) used for sending the
	message.
	\item \texttt{efficiency}: spectral efficiency (in bps/Hz) used
	for sending the message.
	\item \texttt{power}: power (in dBm) of the signal that carries
	the information to be sent.
\end{itemize}
